Polynomial-time Algorithms for Multiple-arm Identification with Full-bandit Feedback

We study the problem of stochastic combinatorial pure exploration (CPE), where an agent sequentially pulls a set of single arms (a.k.a. a super arm) and tries to find the best super arm. Among a variety of problem settings of the CPE, we focus on the full-bandit setting, where we cannot observe the reward of each single arm, but only the sum of the rewards. Although we can regard the CPE with full-bandit feedback as a special case of pure exploration in linear bandits, an approach based on linear bandits is not computationally feasible since the number of super arms may be exponential. In this paper, we first propose a polynomial-time bandit algorithm for the CPE under general combinatorial constraints and provide an upper bound of the sample complexity. Second, we design an approximation algorithm for the 0-1 quadratic maximization problem, which arises in many bandit algorithms with confidence ellipsoids. Based on our approximation algorithm, we propose novel bandit algorithms for the top-k selection problem, and prove that our algorithms run in polynomial time. Finally, we conduct experiments on synthetic and real-world datasets, and confirm the validity of our theoretical analysis in terms of both the computation time and the sample complexity.

==> sec/problem_def.tex <==

\section{Problem Formulation}\label{sec:prob}
\todo{def of ordinary MAB and best arm identification}
Suppose that we have $n$ single arms and the single arms are numbered $1,2,\ldots,n$.
Assume that each arm $e \in[n]$ is associated with a reward distribution $\phi_e$. 
Let $\bm{\theta}^*= (\theta^*_1, \ldots,  \theta^*_n)^{\top} $ denote the vector of expected rewards, where each entry $\theta^*_e= \Exp_{X \sim \phi_e}[{X}]$ denotes the expected reward of arm $e$.
We assume that all reward distributions have R-sub-Gaussian tails for some known constant $R>0$, following standard assumptions of stochastic MABs.
Formally, if $X$ is a random variable drawn from $\phi_e$ for $e \in [n]$,
then, for all $t \in \mathbb{R} $, $X$ satisfies $\Exp[{\exp (tX -t\Exp{X}) }] \leq \exp(R^2t^2/2)$.

We define a {\em decision class} ${\cal M} \subseteq 2^{[n]}$ as a collection of super arms.
Let $K=| {\cal M}|$ be the size of ${\cal M}$.  
For any super arm $M \in {\cal M}$ and  any vector $\theta \in \mathbb{R}^n$,
we define the reward of $M$ in terms of $\theta$ as following:
\begin{align}\label{def:f}
f(\theta, M)=\sum_{e \in M}\theta_e. \notag
\end{align}

We formally define Top-$k$ as follows.
\begin{problem} [Top-$k$] \label{prob:topk}
There are $n$-single arm, where each single arm $e$ is associated with an unknown reward distribution $\phi_e$, with mean $\theta^*_e$.
For any $k \in [n]$, a collection of super arms can be modeled by ${ \cal M}_{{\rm TopK}(k)}= \{M \subseteq 2^{[n]} \mid |M|=k \}$.
At each step we choose a super arm $M \in { \cal M}_{{\rm TopK}(k)}$
and observe the reward of $M$ generated  from unknown distributions.
We aim to identify the best super arm $M^* \in  { \cal M}_{{\rm TopK}(k)}$.
\end{problem}

We also give the definition of pure exploration problem under matroid constraint as follows.
\begin{problem}[Matroid] \label{prob:matroid}
%In a Best-Basis instance $S = (S, M)$, we are given a set $S$ of $n$ single arms. Each arm $e \in S$ is associated with an unknown reward distribution $\phi_e$ with mean $\theta^*_e$.
We are  given a matroid $J= (E,{\cal I})$, where $E=\{1, \ldots, n\}$ is a set of $n$ items (called {\em ground set} ),
and ${\cal I}$ is a family of subsets of $E$ (called the {\em independent sets}).
The weights $w \in \mathbb{R}_{+}^n$ simply sets the weight of $e$ to be the mean of $\phi_e$ for all $e \in E$.
A collection of super arms can be models by ${\cal M}_{\rm Matroid}= \{ M \in {\cal I}\}$.
At each step we choose a basis $M \in {\cal I}$ 
and observe the reward of $M$ generated from unknown distributions.
Our goal is to find a maximum weight basis of the matroid $M^* \in {\cal M}_{\rm Matroid} $.
\end{problem}
The details of definition of a matroid is described in Appendix.
We note that Topk is a special case of a matroid constraint,
since Top-$k$ corresponds to uniform matroids of rank $k$.
%A matroid captures a many classed of combinatorial structures



% Let $M^* = \argmax_{M \in \cM} \sum_{e \in M} \theta^*_e $  denote the optimal member of the decision class ${\cal M}$ that maximizes the sum of expected rewards.
% A player's objective is to identify $M^*$ from ${\cal M}$ by interacting with the following game with the stochastic environment.
% The reward distributions $\{\phi_e \}_{e \in [d]}$ are known to the player.
% The player plays the game over sequence of rounds; in each round $t$,
% she pulls a super arm $M_t \in {\cal M}$ and can observe a whole rewards  $r_t=\sum_{e \in M_t}\theta_e(t)$.
% The game continues until certain stopping condition is satisfied.

We consider the stopping condition known as the {\em fixed confidence} setting in the literature~\cite{}.
In the fixed confidence setting, the player can stop the game at any round.
After the game ends, the player needs to output a super arm ${\tt Out} \in {\cal M}$.
She needs to guarantee that $\Pr[{\tt Out } = M^*] \geq 1-\delta$ for a given confidence parameter $\delta$.
The player's performance is evaluated by her {\em sample complexity}, i.e. the number of samples used by the player.



%\begin{itemize} 
   
  %  \item {  The problem is to find the super arm $\hat{M}^*$ which satisfies $\Pr[(\bm{\chi}_{\sm M^*}-\bm{\chi}_{ \scalebox{0.5} {$\hat{M}^*$}})^{\top} \theta \geq \epsilon] \leq \delta$  }
%\end{itemize}

% ・{\em fixed confidence} setting:
% The learner need to guarantee that $\Pr[{\tt Out}=M^*] \geq 1-\delta$ for given confidence parameta $\delta$. The learner's performance is evaluated by her {\em sample complexity}, i.e. number of pills used by the leaner.\\
% ・{\em fixed budget} setting:
% The leaner need to minimize the {\em probability of error}, which is formally $\Pr[{\tt Out} \neq S^*]$, whithin fixed number $T$ rounds.

We focus on the $(\epsilon,\delta)$-combinatorial pure exploration problem in the fixed confidence setting.
The problem is to design an algorithm to return ${\tt Out} \in {\cal M}$ that satisfies
\begin{align}\label{epsilon-delta}
\Pr[f(\theta^*, M^*)-f(\theta^*, {\tt Out}) \leq \epsilon] \geq 1-\delta. 
\end{align}

We introduce several notations before stating the results.
Let $\Delta(M, M')=f(\theta^*,M )-f(\theta^*,M')$ be the value {\em gap} between two super arms.
Then we denote minimum gap by $\Delta_{\min}= \min_{M \in {\cal M}}\Delta(M^*, M)$.
We also define $\widehat{\Delta}(M, M')=f(\thetahat,M )-f(\thetahat,M')$ as the {\em empirical gap} between two super arms. 

%memo: proposi1 の$K$は改善できる


==> sec/selection.tex <==
\section{Arm Selection Strategy}
In this section, we propose a arm selection policy and derive $\rho^G(\lambda)$ for it.

\begin{theorem}
Let $c_1,\dots,c_d$ be
\begin{align*}
    &c_1 = [\underbrace {1,1,\dots,1}_{k},0,\dots,0]^\top\\
    &c_2 = [0,\underbrace {1,1,\dots,1}_{k},0,\dots,0]^\top\\
    &\vdots\\
    &c_d = [\underbrace {1,1,\dots,1}_{k-1},0,\dots,1]^\top.
\end{align*}
Then $\rho^G((1/d,\dots,1/d)) = \sqrt{d}$
\end{theorem}

\begin{proof}
Let \begin{align*}
B = \sum_{i=1}^d c_i c^\top_i = \frac{1}{d} \begin{bmatrix}
k& (k-1)&\dots&1&0&\dots&0&1&\dots&(k-1)\\
k-1& k& k-1&\dots&1&0&\dots&0&\dots&k-2\\
\vdots& \vdots& \vdots&\vdots&\vdots&\vdots&\vdots&\vdots&\vdots&\vdots\\
k-1& (k-2)&\dots&1&0&\dots&0&2&\dots&k\\
\end{bmatrix}
\end{align*}
Since $B$ is a circulant matrix, $j$-th eigenvalue $\sigma_j$ is
\begin{align*}
\sigma_j &= k + (k-1)\left(\mathrm{e}^{\frac{2\pi i j}{n}}+\mathrm{e}^{\frac{2\pi i j(n-1)}{n}}\right) + (k-2)\left(\mathrm{e}^{\frac{2\pi i (2j)}{n}} + \mathrm{e}^{\frac{2\pi i j(n-2)}{n}}\right) + \dots\\
&= k + \cos\left(2\pi \frac{j}{n}\right) k(k-1)
\end{align*}


\end{proof}
